ID$^3$: Identity-Preserving-yet-Diversified Diffusion Models for Synthetic Face Recognition

Synthetic face recognition (SFR) aims to generate synthetic face datasets that mimic the distribution of real face data, which allows for training face recognition models in a privacy-preserving manner. Despite the remarkable potential of diffusion models in image generation, current diffusion-based SFR models struggle with generalization to real-world faces. To address this limitation, we outline three key objectives for SFR: (1) promoting diversity across identities (inter-class diversity), (2) ensuring diversity within each identity by injecting various facial attributes (intra-class diversity), and (3) maintaining identity consistency within each identity group (intra-class identity preservation). Inspired by these goals, we introduce a diffusion-fueled SFR model termed $\text{ID}^3$. $\text{ID}^3$ employs an ID-preserving loss to generate diverse yet identity-consistent facial appearances. Theoretically, we show that minimizing this loss is equivalent to maximizing the lower bound of an adjusted conditional log-likelihood over ID-preserving data. This equivalence motivates an ID-preserving sampling algorithm, which operates over an adjusted gradient vector field, enabling the generation of fake face recognition datasets that approximate the distribution of real-world faces. Extensive experiments across five challenging benchmarks validate the advantages of $\text{ID}^3$.

==> sec/2_related_work.tex <==
\section{Related Work}

\paragraph{Face Recognition.}
Face Recognition (FR) is the task of matching query imagery to an enrolled identity database. SoTA FR models are trained using margin-based softmax losses~\cite{wang2018cosface, deng2019arcface}  on large-scale web-crawled datasets ~\cite{guo2016ms,zhu2021webface260m}. These datasets encompass three characteristics in common (as mentioned in the introduction): 
(i) sufficient inter-class diversity; (ii) intra-class diversity; (iii) intra-class identity preservation. However, due to the introduction of various regulations restricting the use of authentic face data, 
researchers have switched their attention to synthetic face recognition (SFR). 
We argue that the crux of SFR is to generate a training dataset that inherits the three characteristics above.
%


\noindent\textbf{GAN-based SFR models.}
Most of the deep generative models for synthetic face generation are based on GANs. 
%A number of recent works utilize adversarial losses to train generators for SFR. 
DigiFace~\cite{bae2023digiface} utilizes a digital rendering pipeline to generate synthetic images based on a learned model of facial geometry and attributes. 
SFace~\cite{boutros2022sface} and ID-Net~\cite{kolf2023identity} train a StyleGAN-ADA~\cite{karras2020training} under a class-conditional setting. 
SynFace~\cite{qiu2021synface} extends DiscoFaceGAN~\cite{deng2020disentangled} using synthetic identity mix-up to enhance the intra-class diversity. 
However, the reported results shown by these models show significant performance degradation in comparison to FR trained on real data. 
This performance gap is mainly due to inter-class discrimination and small intra-class diversity in their generated synthetic training datasets. 
%A realistic trade-off between these two characteristics, as we will demonstrate in this paper, is needed to achieve high SFR performance.

\noindent\textbf{Diffusion models for SFR.} 
Recently, Diffusion Models (DMs)~\cite{ho2020denoising, lin2018conditional,song2020denoising} gained attention for both research and industry due to their potential to rival GANs on image synthesis, 
as they are easier to train without stability issues and stem from a solid theoretical foundation. 
%Besides that, they can be conditioned on additional information, and demonstrated impressive results in a wide range of tasks.
%especially in text-to-image generation such as OpenAI’s DALLE 2~\cite{ramesh2022hierarchical}, LDM~\cite{Rombach_2022_CVPR}, and Google’s Imagen~\cite{dhariwal2021diffusion}.
Among SFR diffusion models, IDiff-Face~\cite{boutros2023idiff} achieves SoTA performance. On the basis of a diffusion model, it incorporates Contextual Partial Dropout to generate diverse intra-class images. 
However, IDiff-Face fails to regularize the relationship among different identities.
%the identity consistency of the dropped-out embeddings.


==> sec/4_experiments.tex <==
\section{Experiments}
\subsection{Datasets}

% \begin{wrapfigure}{r}{.5\textwidth}
% % \vspace{-0.15in}
% \centering
% \includegraphics[scale=0.4]{Fig/Fig_3.png}
% \caption{Fine Annotation in Else~\cite{fuhl2016else}}
% \vspace{-0.15in}
% \label{FA}
% \end{wrapfigure}


% \begin{figure}[htbp]
%     % \vspace{-0.25in}
%     \begin{minipage}{.5\textwidth}
%          There are several publicly available iris datasets \cite{fuhl2015excuse}\cite{fuhl2016else}\cite{garbin2020dataset}\cite{fuhl2021teyed}\cite{tonsen2016labelled}\cite{fuhl2016pupilnet}\cite{fuhl2017pupilnet}\cite{kim2019nvgaze} that have been established to aid research and algorithm development. Some datasets \cite{fuhl2021teyed}\cite{tonsen2016labelled} approximate the boundary with ellipses, which introduces geometrical bias. We meticulously annotate an iris detection dataset ElSe \cite{fuhl2016else}. Compared with other iris segmentation datasets \cite{garbin2020dataset}, the image quality of our finely annotated data set is worse and can simulate more extreme environments in reality. The figure provides a visual representation of the dataset, showcasing the challenges present in captured iris images due to factors like lens distortion. As a result, the actual iris shapes obtained through our capture process deviate from the ideal elliptical shape. Additionally, the dataset contains various types of noise that pose significant challenges during iris image analysis.\par
%     \end{minipage}
%     \begin{minipage}{.5\textwidth}
%     % \vspace{0.1in}
%     \centering
%     \includegraphics[scale=0.4]{Fig/Fig_3.png}
%     \caption{Fine annotation in Else\cite{fuhl2016else}}
%     \label{dataset}
%     \end{minipage}
%     \vspace{-0.15in}
% \end{figure} 


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{Fig/sample_fea.pdf}
    \caption{\small An illustration of ID-preserving sampling algorithm.}
    \label{fig:sample_fea}
    \vspace{-0.1in}
\end{figure}  

 
There are several publicly-available\textit{ iris datasets}~\cite{fuhl2015excuse,fuhl2016else,garbin2020dataset,fuhl2021teyed,tonsen2016labelled,fuhl2016pupilnet,
fuhl2017pupilnet,kim2019nvgaze} that have been established to aid research and algorithm development. 
Among them \cite{fuhl2021teyed,tonsen2016labelled} approximate the iris boundary by ellipses, 
which may introduce geometrical biases.
To this end, we have meticulously annotated an iris detection dataset, Else~\cite{fuhl2016else},
making the images in it worse in quality to simulate more extreme scenes in reality compared to other iris segmentation datasets \cite{garbin2020dataset}.
% Compared with other iris segmentation datasets \cite{garbin2020dataset}, 
% the image quality of our finely annotated dataset is worse and can simulate more extreme environments in reality. 
\figureautorefname{~\ref{fig:toydata}} provides a visual representation of the dataset, 
showcasing the challenges present in captured iris images due to factors like lens distortion. 
As a result, the actual iris shapes obtained through our capture process deviate from the ideal elliptical shape. 
% Additionally, the dataset contains various types of noise that pose significant challenges during iris image analysis.
Various types of noise in the datasets also bring great challenges to iris image analysis.


We conduct extensive experiments to evaluate our proposed approach on multiple widely used datasets, including OpenEDS~\citep{openeds}, LPW (Labelled Pupils in the Wild)~\cite{LPW}, and Dikablis~\cite{fuhl2022teyed}. 
These datasets provide diverse ranges of real-world scenarios and variations in imaging conditions.
We also curated our own annotated dataset specifically tailored to assess the performance of our method. 
% By testing our approach on these datasets, 
% we are able to demonstrate its effectiveness and robustness across different datasets with varying characteristics and challenges.

Furthermore, to increase the diversity of training data and expand the dataset, we use conventional data augmentation techniques such as random rotation, translation, scaling, and horizontal flipping. 
We also apply gamma correction to the image during the preprocessing stage.





\subsection{Implementation Details}

All experimental settings, including data preprocessing, network architecture, and hyperparameters, were kept the same for a fair comparison.

Our proposed first stage is based on a similar architecture to YOLOv3~\cite{yolov3} for object detection, which enables us to localize and identify regions of interest in images efficiently. By using a smaller network structure, we can effectively locate the sub-region of interest. We achieve this by cutting the original darknet and obtaining a subnetwork with only 43.13M FLOPs of computation. After completing the first stage, we transform all subimages of interest into $96\times96$ images to serve as input to the segmentation model. 
% This approach allows us to segment the regions of interest and achieve high-quality results accurately.
In the second stage, we utilize the lightweight segmentation network structures DeepVOG~\cite{yiu2019deepvog} and EyeNet-L~\cite{feng2022real} as the backbone network for segmentation, which we refer to as Ours(D) and Ours(E), respectively. The input size of the network is standardized to $96\times96$, and the output category of network segmentation is set to $K=4$ categories (Pupil, Iris, Eye and Background). To demonstrate the independence of our framework from the segmented network structure, we use various classic iris segmentation networks as the backbone in Table \ref{tab8}, with input and output consistent with Ours(D). Due to the sub-graph positioning, our framework has a much smaller computational load than that of full-image input, even with the same segmentation network structure.

Our uncertainty estimation header utilizes the same upsampling and downsampling modules as the backbone network.  
It consists of one downsampling layer and two upsampling layers, with skip connections to obtain the corresponding outputs from the backbone at each level. By incorporating these skip connections, our uncertainty estimation network can leverage the rich feature representations extracted by the backbone network.  The downsampling layer reduces the spatial dimensions of the input, capturing high-level contextual information.  The subsequent upsampling layers recover the spatial resolution, enabling fine-grained uncertainty estimation at each pixel. This architecture design ensures that our uncertainty estimation network can effectively capture both global and local information from the backbone network.  The skip connections facilitate information flow and enable the network to leverage hierarchical features for more accurate uncertainty estimation.  Overall, this design choice contributes to the robustness and reliability of our uncertainty estimation framework.



\subsection{Results}


\subsubsection{Segmentation}



\tableautorefname{~\ref{tab:openeds_res}} reports the segmentation results of different methods on OpenEDS dataset,
it shows 
% The results obtained on the OpenEDS dataset demonstrate 
that our approach outperforms the state-of-the-art DenseElNet method with significant improvement and up to %an average increase of 
$3.7\%$ for the average MIoU (Mean Intersection over Union) scores while utilizing only 0.3\% of the computational resources. 
This improvement is attributed to our method's ability to exclude irrelevant noise during the processing, leading to a more efficient and accurate model. 
These findings highlight the significant advancements of our approach in the field of image semantic segmentation.

\begin{table}[t]
    \centering
    \caption{Segmentation results (MIoU) on OpenEDS and computation of the segmentation backbone.}
    \label{tab:openeds_res}
    \vspace{-0.1in}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l | c | c | r} \toprule %[1.5pt]    %\hline
        Methods & Iris MIoU & Pupil MIoU & \multicolumn{1}{c}{FLOPs}\\  \hline  % \hline\hline
        DeepVOG~\cite{kothari2021ellseg}  & N/A & 89.1 & 3.50G\\    % \hline
        RITnet~\cite{kothari2021ellseg}  & 91.4 & 95.0 & 16.57G\\  % \hline
        DenseElNet~\cite{kothari2021ellseg}  & 92.1 & 95.4 & 42.58G\\  % \hline
        Ours(E)  & 97.9 & 97.0 & \textbf{91.39M}\\  % \hline
        Ours(D)  & \textbf{98.3} & \textbf{97.3} & 125.85M\\ 
        \bottomrule %[1.5pt] %\hline
    \end{tabular}
   }
\end{table}

In addition, we also evaluate the performance of our method on other datasets, and the results are presented in \tableautorefname{~\ref{tab:segments}}. 
The configurations of DeepVOG~\cite{yiu2019deepvog} and RITnet~\cite{chaudhary2019ritnet} used here are consistent with the original training settings in their respective papers.
It demonstrates that our proposed subregion-based segmentation framework achieves better or equivalent results using only a segmentation network with a small amount of computation.

\begin{table}[t]
    \centering
    \caption{Segmentation results (i.e., MIoU for Iris and Pupil) on Else, Dikablis, and LPW datasets.} 
    \label{tab:segments}
    \vspace{-0.1in}
    \begin{tabular}{l|ll|ll|ll}  \toprule
    \multicolumn{1}{c|}{}        & \multicolumn{2}{c|}{Else}                             & \multicolumn{2}{c|}{Dikablis}                         & \multicolumn{2}{c}{LPW}                              \\ \hline
    \multicolumn{1}{c|}{Methods} & \multicolumn{1}{c}{Iris} & \multicolumn{1}{c|}{Pupil} & \multicolumn{1}{c}{Iris} & \multicolumn{1}{c|}{Pupil} & \multicolumn{1}{c}{Iris} & \multicolumn{1}{c}{Pupil} \\ \hline
    DeepVOG                      & 93.0                     & 87.0                       & 91.1                     & \textbf{94.2}              & 79.7                     & 83.9                      \\
    RITnet                       & 93.7                     & \textbf{88.7}              & 91.6                     & 94.7                       & 86.7                     & 86.3                      \\
    Ours (E)                     & 93.1                     & 83.0                       & 89.2                     & 91.6                       & 88.9                     & 93.1                      \\
    Ours (D)                     & \textbf{95.1}            & 87.6                       & \textbf{91.7}            & \textbf{94.2}              & \textbf{90.1}            & \textbf{93.5}             \\ \bottomrule
    \end{tabular}
\end{table}

% \begin{table}[h]
%     \begin{minipage}{.5\textwidth}
%         \centering
%         \caption{Segmentation results (MIoU) on Else.}
%         \label{tab2}
%         \begin{tabular}{l | c | c} \toprule %[1.5pt] \hline
%         Methods & Iris MIoU & Pupil MIoU\\ \hline % \hline
%         DeepVOG  & 93.0 & 87.0\\  % \hline
%         RITnet   & 93.7 & \textbf{88.7}\\ % \hline
%         Ours(E)  & 93.1 & 83.0\\          % \hline
%         Ours(D)  & \textbf{95.1} & 87.6\\  \bottomrule %[1.5pt] \hline
%         \end{tabular}
%     \end{minipage}
%     \begin{minipage}{.5\textwidth}
%         \centering
%         \caption{Segmentation results (MIoU) on Dikablis.}  
%         \label{tab3}
%         \begin{tabular}{l | c | c}       \toprule %[1.5pt]  \hline
%         Methods & Iris MIoU & Pupil MIoU\\ \hline % \hline
%         DeepVOG  & 91.1 & \textbf{94.2}\\  % \hline
%         RITnet  & 91.6 & 94.7\\   % \hline
%         Ours(E)  & 89.2 & 91.6\\  % \hline
%         Ours(D)  & \textbf{91.7} & \textbf{94.2}\\  \bottomrule %[1.5pt] \hline
%         \end{tabular}
%     \end{minipage}
% \end{table} 

% \begin{table}[h]
% \caption{Segmentation results (MIoU) on LPW.}
% \begin{center}
% \begin{tabular}{l | c | c}
% \toprule[1.5pt]
% \hline
% Methods & Iris MIoU & Pupil MIoU\\
% \hline
% % \hline
% DeepVOG  & 79.7 & 83.9 \\ 
% % \hline
% RITnet  & 86.7 & 86.3\\ 
% % \hline
% Ours(E)  & 88.9 & 93.1\\ 
% % \hline
% Ours(D)  & \textbf{90.1} & \textbf{93.5}\\ 
% \bottomrule[1.5pt]
% \hline
% \end{tabular}
% \end{center}
% \label{tab4}
% \end{table}

\subsubsection{Uncertainty Estimation}

To evaluate the performance of our uncertainty-based rejection approach on erroneous samples in two scenarios: 
within the same dataset and across different datasets. 
In the same dataset scenario, we mainly simulate the effects of factors such as image blurriness and noise on model performance. In the cross-dataset scenario, we mainly simulate the performance degradation caused by domain gaps.
In order to make a fair comparison, we only use the uncertainty method in the following framework, and DeepVOG is used by the backbone.

\begin{table*}[thp]
    \centering
    \caption{The MIoU after removing images with high uncertainty (models trained on Else and evaluated on Else).}
    \label{tab5}
    \vspace{-0.1in}
    % \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l | c | c | c | c | c | c} \toprule %[1.5pt] \hline
        Methods & 0 & 0.01 & 0.02 & 0.03 & 0.04 & 0.05\\ \hline
        % QC-MC Dropout   & 81.85 & 82.18(0.33) & 82.35(0.50) & 82.54(0.69) & 82.62(0.77) & 82.72(0.87)\\
        Ensemble & 86.96 & 87.11 $\pm$ \textbf{0.15} & 87.14 $\pm$ 0.18 & 87.21 $\pm$ 0.25 & 87.26 $\pm$ 0.30 & 87.33 $\pm$ 0.37\\
        BiTrans  & 86.62 & 86.75 $\pm$ 0.13 & 86.80 $\pm$ 0.18 & 86.90 $\pm$ 0.28 & 86.97 $\pm$ 0.35 & 87.10 $\pm$ 0.48\\
        EvPSNet  & 87.21 & 87.28 $\pm$ 0.07 & 87.28 $\pm$ 0.07 & 87.45 $\pm$ 0.24 & 87.48 $\pm$ 0.27 & 87.48 $\pm$ 0.27\\
        Ours(D)  & \textbf{89.17} & \textbf{89.32 $\pm$ 0.15} & \textbf{89.39 $\pm$ 0.22} & \textbf{89.46 $\pm$ 0.29} & \textbf{89.68 $\pm$ 0.51} & \textbf{89.72 $\pm$ 0.55}\\ \bottomrule %]1.5pt]\hline
    \end{tabular}
    % }
\end{table*}

\begin{table*}[thp]
    \centering
    \caption{The MIoU after removing images with high uncertainty (models trained on Else and evaluated on OpenEDS).}
    \label{tab6}
    \vspace{-0.1in}
    \begin{tabular}{l | c |c| c| c| c| c} \toprule %[1.5pt] \hline
        Methods & 0 & 0.01 & 0.02 & 0.03 & 0.04 & 0.05\\ \hline
        % QC-MC Dropout & 60.00 & 60.09(0.09) & 60.17(0.17) & 60.21(0.21) & 60.25(0.25) & 60.31(0.31)\\
        Ensemble & 71.37 & 71.49 $\pm$ 0.12 & 71.62 $\pm$ 0.25 &  71.73 $\pm$ 0.36 & 71.84 $\pm$ 0.47 & 71.93 $\pm$ 0.56\\
        BiTrans  & 75.73 & 75.87 $\pm$ 0.14 & 75.99 $\pm$ 0.26 &  76.10 $\pm$ 0.37 & 76.18 $\pm$ 0.45 & 76.27 $\pm$ 0.54\\
        EvPSNet  & 76.46 & 76.61 $\pm$ 0.15 & 76.73 $\pm$ 0.27 &  76.79 $\pm$ 0.33 & 76.86 $\pm$ 0.40 & 76.90 $\pm$ 0.44\\
        Ours(D)  & \textbf{86.25} &	\textbf{86.56 $\pm$ 0.31} &	\textbf{86.76 $\pm$ 0.51} &	\textbf{86.89 $\pm$ 0.64} &	\textbf{87.02 $\pm$ 0.77} &	\textbf{87.15 $\pm$ 0.90}\\ \bottomrule%[1.5pt] \hline
    \end{tabular}
\end{table*}

We collect all images from the dataset and rank them based on the confidence scores generated by the uncertainty estimation model. By filtering out a portion of the images according to the ranking, our system achieves better segmentation performance. 
To ensure fairness, all methods are evaluated based on the segmented MIoU. 
As demonstrated in Table \ref{tab5} and Table \ref{tab6}, the images selected by our proposed uncertainty evaluation method outperform those selected manually. This indicates that our framework is effective in evaluating the results of segmentation models for segmentation tasks.

% To facilitate the task, we have devised a procedure involving three individuals. Initially, Person 1 selects a subset of samples from the dataset in Situation 1, while Person 2 independently reviews and identifies potential errors among the selected samples. This process is repeated in Situation 2 with a different subset of samples. In case of any discrepancies or disagreements between Person 2's selections in both situations, Person 3, acting as an expert reviewer, makes the final decision. By incorporating the judgments of multiple individuals and an expert reviewer, we aim to ensure a comprehensive and reliable assessment of potential errors.

\subsection{Downstream Task}

The purpose of this study is to apply the uncertainty method in practical scenarios and examine its effectiveness in such settings. 
To achieve this, we conducted experiments in the context of gaze estimation.
We utilized the DeepVog method~\cite{kothari2021ellseg} to construct the eyeball model. Through experimentation, we obtained the experimental results shown in Table x, which revealed the significant benefits of the uncertainty method for gaze estimation.


\begin{table}[h]
    \centering
    \caption{Gaze Estimation with uncertainty method}
    \label{tab6}
    \vspace{-0.1in}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l   | c| c| c| c}  \toprule %[1.5pt] \hline
        Methods & Ensemble & BiTrans & EvPSNet & Our(D)\\ \hline
        Pure   & 3.81 & 3.92 & 4.30 & 2.90\\  %\hline
        Uncertainty & \textbf{3.71} & \textbf{3.83} & \textbf{4.21} & \textbf{2.75} \\ \bottomrule %[1.5pt] \hline
    \end{tabular}
    }
\end{table}


\section{Ablation Study}



\subsection{Different objective functions}
We conduct experimental comparisons of the two optimization objectives proposed (Eq.~\eqref{loss} and Eq.~\eqref{uploss}) in this paper. From the results presented in Table \ref{tab7}, it can be observed that both optimization objectives yield improvements. The results obtained from each stage of Table \ref{tab7} demonstrate that the upgraded loss function provides a more accurate estimation of the uncertainty associated with the segmentation results.
% However, in comparison, the distance-based method outperforms the original optimization objective in terms of effectiveness.

\begin{table*}[htp]
    \centering
    \caption{Comparisons of the two optimization objectives (models trained and evaluated on Else).}
    \label{tab7}
    \vspace{-0.1in}
    \begin{tabular}{c |c| c| c| c| c| c} \toprule %[1.5pt] \hline
        Objective Loss & 0 & 0.01 & 0.02 & 0.03 & 0.04 & 0.05\\  \hline
        Original in Eq.~(2) %$\mathcal{L}_{i,j}$ in (2) 
        & 89.17 & 89.20 $\pm$ 0.03 &	89.30 $\pm$ 0.13 &	89.32 $\pm$ 0.15 & 89.36 $\pm$ 0.19 &	89.37 $\pm$ 0.20 \\
        Surrogate in Eq.~(8) % $\mathcal{L}_{i,j}$ in (8) 
        & 89.17 & \textbf{89.32 $\pm$ 0.15} & \textbf{89.39 $\pm$ 0.22} & \textbf{89.46 $\pm$ 0.29} & \textbf{89.68 $\pm$ 0.51} & \textbf{89.72 $\pm$ 0.55}\\ \bottomrule %[1.5pt] \hline
    \end{tabular}
\end{table*}

% Our approach, proposed in this paper, is a backbone-agnostic method that is applicable across different backbone architectures. We evaluated our method using a larger-scale backbone and compared its performance. Remarkably, even with an increase in Flops, our model achieved further improvements in performance. This demonstrates the effectiveness and versatility of our approach across different backbone configurations.

\subsection{Backbone networks}
The subregion-based segmentation framework of our method %proposed in our paper is independent of 
is agnostic to the backbone architecture.
% and can be applied to different backbone architectures. 
Therefore, we evaluate our method and compare its performance using backbones of different sizes and report the results in Table \ref{tab8}.
In this experiment, we replace the segmented backbone while keeping the structure of the sub-region detection as it is. 
It is noteworthy that as the FLOPs in the backbone calculation increase, our framework achieves further improvement in the final segmentation results. This demonstrates the effectiveness and generalizability of our method across different backbone network configurations.


% \hline
% Backbone & OpenEDS & Else & Dikablis & LPW & Params & FLOPs \\
% \hline
% Ours(E) & 96.5 & 88.12 & 90.4  & 91.0 & \textbf{66500} &	\textbf{91.39M}\\	
% \hline
% Ours(D) & 97.1 & -89.5 & 92.9 & 91.8 & 232316 &	125.85M\\
% \hline

% Bisev1 \cite{yu2018bisenet}  & 97.1 & 91.69	& 93.4	& 92.3 & 13259140 &  493.05M\\ 
% \hline
% % Bisev2 \cite{yu2021bisenet} & 97.1 & 91.31 &	93.2 &	88.2 & 3341812	& 429.64M \\
% % \hline
% DenseElNet~\cite{kothari2020ellseg} & \textbf{97.7} & \textbf{93.21} &	\textbf{94.2} &	\textbf{93.6} & 2181470 & 1.53G\\ 

\begin{table*}[thp]
    \centering
    \caption{Results of subregion-based segmentation framework in different backbones. All network inputs are $96 \times 96$.}
    \label{tab8}
    \vspace{-0.1in}
    \begin{tabular}{l|c|c|c|c|r|r} \toprule %\hline
        \multicolumn{1}{c|}{Backbone}        & OpenEDS       & Else          & Dikablis      & LPW  & \multicolumn{1}{c|}{\# of Params} & \multicolumn{1}{c}{FLOPs} \\ \hline
        Ours (E)                             & 96.5          & 85.8          & 90.4          & 91.0 & \textbf{66,500}                   & \textbf{91.39 M} \\
        Ours (D)                             & 97.1          & 89.2          & 92.9          & 91.8 & 232,316                           & 125.85 M         \\
        Bisev1~\cite{yu2018bisenet}          & 97.1          & 90.4          & 93.4          & 92.3 & 13,259,140                        & 493.05 M         \\
        % Bisev2 \cite{yu2021bisenet}        & 97.1          & 88.9          &93.2           & 88.2 & 3,341,812	                        & 429.64M \\ % \hline
        DenseElNet\cite{kothari2020ellseg} & \textbf{97.7} & \textbf{91.3} & \textbf{94.2} & 93.6 & 2,181,470                           & 1.53 G           \\ \bottomrule
    \end{tabular}
\end{table*}

\begin{table*}[thp]
    \centering
    \caption{Results of subregion-based segmentation framework in different backbones. All network inputs are $96 \times 96$.}
    \label{tab8}
    \vspace{-0.1in}
    \begin{tabular}{l |c| c| c| c| c| c} \toprule %[1.5pt] \hline
        Backbone & OpenEDS & Else & Dikablis & LPW & \# of Params & FLOPs \\ \hline
        Ours(E) & 96.5 & 85.8 & 90.4  & 91.0 & \textbf{66,500} &	\textbf{91.39M}\\%\hline
        Ours(D) & 97.1 & 89.2 & 92.9 & 91.8 & 232,316 &	125.85M\\  %\hline
        Bisev1 \cite{yu2018bisenet}  & 97.1 & 90.4	& 93.4	& 92.3 & 13,259,140 &  493.05M\\  %\hline
        % Bisev2 \cite{yu2021bisenet} & 97.1 & 88.9 &	93.2 &	88.2 & 3341812	& 429.64M \\ % \hline
        DenseElNet~\cite{kothari2020ellseg} & \textbf{97.7} & \textbf{91.3} &	\textbf{94.2} &	\textbf{93.6} & 2,181,470 & 1.53G\\  \bottomrule %[1.5pt] \hline
    \end{tabular}
\end{table*}



We conduct a comprehensive comparison between our method's uncertainty estimation and segmentation performance on both the entire image and sub-regions. Our method consistently outperforms the other regardless of the proportion of data removed according to the uncertainty scores estimated by our framework.

\begin{table*}[thp]
    \centering
    \caption{Comparison between our method's uncertainty estimation and segmentation performance on both the entire image and sub-regions.}
    \label{tab9}
    \vspace{-0.1in}
    \begin{tabular}{l |c| c| c| c| c |c} \toprule %[1.5pt] \hline
        Methods & 0 & 0.01 & 0.02 & 0.03 & 0.04 & 0.05\\  \hline
        Entire image  & 86.97 & 87.09 $\pm$ 0.12 & 87.36 $\pm$ 0.39 &	87.48 $\pm$ 0.51 &	87.57 $\pm$ 0.60 &	87.77 $\pm$ 0.80\\ %epoch 7 \hline
        Ours(D) & 89.17 & \textbf{89.32 $\pm$ 0.15} & \textbf{89.39 $\pm$ 0.22} & \textbf{89.46 $\pm$ 0.29} & \textbf{89.68 $\pm$ 0.51} & \textbf{89.72 $\pm$ 0.55}\\ \bottomrule %[1.5pt] \hline
    \end{tabular}
\end{table*}

==> sec/Checklist.tex <==

\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As shown in the abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As shown in the conclusion.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As shown in the Appendix A and B.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As shown in the experiment and appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As shown in the experiments and appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As shown in the experimental tables.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As shown in the experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The creators or original owners of assets (e.g., code, data, models), used in the paper, are properly credited. The license and terms of use are explicitly mentioned and properly respected.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}




